SkiLD: Unsupervised Skill Discovery Guided by Factor Interactions

Unsupervised skill discovery carries the promise that an intelligent agent can learn reusable skills through autonomous, reward-free environment interaction. Existing unsupervised skill discovery methods learn skills by encouraging distinguishable behaviors that cover diverse states. However, in complex environments with many state factors (e.g., household environments with many objects), learning skills that cover all possible states is impossible, and naively encouraging state diversity often leads to simple skills that are not ideal for solving downstream tasks. This work introduces Skill Discovery from Local Dependencies (Skild), which leverages state factorization as a natural inductive bias to guide the skill learning process. The key intuition guiding Skild is that skills that induce <b>diverse interactions</b> between state factors are often more valuable for solving downstream tasks. To this end, Skild develops a novel skill learning objective that explicitly encourages the mastering of skills that effectively induce different interactions within an environment. We evaluate Skild in several domains with challenging, long-horizon sparse reward tasks including a realistic simulated household robot domain, where Skild successfully learns skills with clear semantic meaning and shows superior performance compared to existing unsupervised reinforcement learning methods that only maximize state coverage.

==> sections/04_theory.tex <==
\section{Sample Complexity of Graph Dependency Skill Learning}
% This work introduces hierarchies guided by local causal graphs. Recent work by ~\citet{FAC paper} has drawn a connection between local causality and the normality assumption in actual causality, which offers a set-based analysis of causal relationships. This allows us to categorize the interaction-based hierarchical RL algorithm proposed in this work along with other object-based skill hierarchies based on the degree to which they leverage, often implicitly, local causal relationships. 

Policies that leverage state-specific graph dependencies can exploit the dynamics properties that are often present in this structure to learn more efficiently. In particular~\citet{bertsekas2015dynamic} proves that value iteration converges in $|\mathcal S|$ steps, where the cost of each policy iteration step is $|\mathcal S||\mathcal A|M$: the cost of updating each state ($|\mathcal S|$) with each action $|\mathcal A|$ and subsequent transition dynamics, where $M$ is number of states reachable in a single transition. For skill learning, we can replace $|\mathcal S|$ \az{?}

% Proof of causal controllability: Assuming that the interaction graphs hold and there are no excess graphs, any state is reachable. The degree of uncontrollability is proportional to the degree to which other graphs occur mid-trajectory.\\

